Energy-Based Policy Orchestration

Hierarchical control scales robot behavior by separating task-level planning from low-level control. In dynamic, high-dimensional tasks, however, a fixed planner-to-policy interface can fail when contacts, balance, or disturbances evolve faster than high-level policy updates. Execution therefore requires choosing not only which low-level policy to run, but also which policy-specific goal should be given to it. We formulate this problem as policy orchestration: runtime selection of a policy-goal pair that is likely to remain feasible while tracking the planner target. We develop EPO, an energy-based policy orchestrator for modular goal-conditioned policy families. For each policy, EPO learns a composite energy over low-level goals, where lower energy corresponds to higher feasibility and more accurate target realization. At runtime, EPO refines each policy's goal and executes the lowest-energy policy-goal pair. Because energies are policy-specific, new policies can be incorporated by learning their own energy models, without retraining the existing policies or a centralized scheduler. In simulation, EPO improves the empirical precision-robustness trade-off by refining policy-specific goals before selectively switching among policies based on energy scores. We further demonstrate sim-to-real deployment of the same frozen policies and energy models on real humanoid loco-manipulation tasks. Project website: https://yewr.github.io/epo

==> app/app_exp_6_real_world.tex <==
\subsection{Real-world experiments}
\label{app:exp-real}

\subsubsection*{Hardware and infrastructure}

Real-world experiments are conducted on the Unitree G1 humanoid. The
deployed system runs the low-level policy at $50$~Hz and uses the same
goal-command interface as in simulation. EPO runs asynchronously with the
low-level policy-control loop: the policy continues executing the most
recent selected policy--command pair while the energy-based optimizer
computes the next one. Unless otherwise stated, the hardware experiments
use the same runtime settings as simulation, including the 10~Hz EPO
orchestration rate, three command-refinement steps, the consistency
floor, and the fixed policy-transition cost $c_{\mathrm{sw}}=0.2$.
Safety checks are enforced by the deployment stack and terminate
execution when joint, velocity, contact, or body-pose constraints are
violated.

\subsubsection*{Task protocols and success criteria}

We evaluate real-world performance on three teleoperated
loco-manipulation tasks: walking to pick up an object, pushing a chair,
and carrying a box with both hands. A human operator provides task-level
commands, while EPO selects the low-level policy--command pair. The tasks
are designed to require different combinations of locomotion, balance,
end-effector tracking, contact-rich interaction, and transitions between
locomotion and manipulation.

\paragraph{Walk and pick.}
The robot starts away from the target object, walks toward it, transitions
to a manipulation posture, and reaches down to pick up or grasp the
object. This task tests whether the controller can move from locomotion
to precise standing manipulation without losing balance. A trial is
successful if the robot reaches the object, completes the pick-up
interaction, and remains standing without manual recovery.

\paragraph{Push chair.}
The robot pushes a chair across the floor while maintaining balance and
task progress. This task introduces sustained external contact and
requires the controller to remain robust to changes in contact force as
the chair starts moving. A trial is successful if the robot moves the
chair to the target region without falling, losing sustained contact, or
requiring manual reset.

\paragraph{Carry box.}
The robot carries a box with both hands while walking over a flat indoor
surface. This task requires coordinated bimanual tracking while the base
continues to move. A trial is successful if the robot transports the box
to the target region without falling, dropping the box, or requiring
operator intervention.

An intervention is counted whenever the operator or experimenter must
manually stop, reset, physically support, or reposition the robot or
object in order to continue the trial. A fall is counted when the robot
triggers the deployment stack's fall or safety termination condition.

\subsubsection*{Detailed per-task results}

\begin{table}[t]
\centering
\caption{Detailed real-world results by task. Success is reported as
successful trials over total trials. Interventions count manual resets,
physical support, or object repositioning required to continue a trial.}
\label{tab:app-real-results}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{llcccc}
\toprule
Task & Method & Success / trials & Falls & Interventions & Time \\
\midrule
Walk and pick & $\pi_{\rm gen}$   & TODO & TODO & TODO & TODO \\
Walk and pick & $\pi_{\rm gen}^R$ & TODO & TODO & TODO & TODO \\
Walk and pick & EPO              & TODO & TODO & TODO & TODO \\
\midrule
Push chair    & $\pi_{\rm gen}$   & TODO & TODO & TODO & TODO \\
Push chair    & $\pi_{\rm gen}^R$ & TODO & TODO & TODO & TODO \\
Push chair    & EPO              & TODO & TODO & TODO & TODO \\
\midrule
Carry box     & $\pi_{\rm gen}$   & TODO & TODO & TODO & TODO \\
Carry box     & $\pi_{\rm gen}^R$ & TODO & TODO & TODO & TODO \\
Carry box     & EPO              & TODO & TODO & TODO & TODO \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection*{Representative failure cases}

We record representative failure cases for each method. Fixed-policy
failures typically arise when a task moves outside the policy's reliable
operating region. The general policy can track manipulation commands more
precisely but is more sensitive to contact disturbances and unstable
postures. The robustness-oriented policy is more tolerant to pushes and
contact but can sacrifice manipulation precision. EPO reduces these
failure modes by switching policies and refining commands at runtime, but
it can still fail when perception, contact geometry, or the commanded
motion falls outside the feasible region of the entire policy family.

% \subsubsection*{Supplementary video index}

% A complete video index is provided in the supplementary material. The
% index maps each real-world task to the corresponding trial videos,
% including successful trials and representative failures.


